S2R: Exploring a Double-Win Transformer-Based Framework for Ideal and Blind Super-Resolution

Nowadays, deep learning based methods have demonstrated impressive performance on ideal super-resolution (SR) datasets, but most of these methods incur dramatically performance drops when directly applied in real-world SR reconstruction tasks with unpredictable blur kernels. To tackle this issue, blind SR methods are proposed to improve the visual results on random blur kernels, which causes unsatisfactory reconstruction effects on ideal low-resolution images similarly. In this paper, we propose a double-win framework for ideal and blind SR task, named S2R, including a light-weight transformer-based SR model (S2R transformer) and a novel coarse-to-fine training strategy, which can achieve excellent visual results on both ideal and random fuzzy conditions. On algorithm level, S2R transformer smartly combines some efficient and light-weight blocks to enhance the representation ability of extracted features with relatively low number of parameters. For training strategy, a coarse-level learning process is firstly performed to improve the generalization of the network with the help of a large-scale external dataset, and then, a fast fine-tune process is developed to transfer the pre-trained model to real-world SR tasks by mining the internal features of the image. Experimental results show that the proposed S2R outperforms other single-image SR models in ideal SR condition with only 578K parameters. Meanwhile, it can achieve better visual results than regular blind SR models in blind fuzzy conditions with only 10 gradient updates, which improve convergence speed by 300 times, significantly accelerating the transfer-learning process in real-world situations.

==> experi.tex <==

% \begin{figure}
%     \centering
%     \subfigure[Barbara]
%     {
%     \begin{minipage}[b]{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{processed barbara_line.png}
%         \label{fig:proposed_barbara_line}
%     \end{minipage}
%     }
%     \subfigure[CARN]
%     {
%     \begin{minipage}[b]{.18\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{crop_resizebarbara_CARN.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_IMDN_patch.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_gt_patch.png}
        
%         \label{fig:training_recipe}
        
%     \end{minipage}
%     }
%     \subfigure[IMDN]
%     {
%     \begin{minipage}[b]{.18\linewidth}
%         \centering
%         % \includegraphics[width=0.3\linewidth]{CARN_bar_patch.png}
%         \includegraphics[width=\linewidth]{crop_resizebarbara_IMDN.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_gt_patch.png}
        
%         \label{fig:training_recipe}
        
%     \end{minipage}
%     }

%     \subfigure[SwinIR-light]
%     {
%     \begin{minipage}[t]{.18\linewidth}
%         \centering
%         % \includegraphics[width=\linewidth]{CARN_bar_patch.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_IMDN_patch.png}
%         \includegraphics[width=\linewidth]{crop_resizebarbara_SwinIR.png}
       
%         \label{fig:training_recipe}
        
%     \end{minipage}
%     }
%     \subfigure[ELAN-light]
%     {
%     \begin{minipage}[t]{.18\linewidth}
%         \centering
%         % \includegraphics[width=\linewidth]{CARN_bar_patch.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_IMDN_patch.png}
%         \includegraphics[width=\linewidth]{crop_resizebarbara_elan.png}
       
%         \label{fig:training_recipe}
        
%     \end{minipage}
%     }
%     \subfigure[Ours]
%     {
%     \begin{minipage}[t]{.18\linewidth}
%         \centering
%         % \includegraphics[width=\linewidth]{CARN_bar_patch.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_IMDN_patch.png}
%         \includegraphics[width=\linewidth]{crop_resizebarbara_sibsr.png}
       
%         \label{fig:training_recipe}
        
%     \end{minipage}
%     }
%     \subfigure[GT]
%     {
%     \begin{minipage}[b]{.18\linewidth}
%         \centering
%         % \includegraphics[width=\linewidth]{CARN_bar_patch.png}
%         % \includegraphics[width=0.3\linewidth]{barbara_IMDN_patch.png}
%         \includegraphics[width=\linewidth]{crop_resizebarbara_gt.png}
       
%         \label{fig:training_recipe}
        
%     \end{minipage}
    
%     }
%     \label{barbara}
%     % \includegraphics[width=\textwidth]{training_recipe.pdf}
% \end{figure}


==> intro.tex <==
\section{Introduction}
Super-Resolution (SR) is proposed to increase the resolution of low-quality images and enhance their clarity. As a fundamental low-level vision task, single image super-resolution (SISR), which aims to recover plausible high-resolution (HR) images from their counterpart low-resolution (LR) images, has attracted increasing attention. With the remarkable success of convolutional neural networks (CNNs), various deep learning based methods with different network architectures and training strategies have been proposed for SISR and achieved state-of-the-art (SOTA) results. Most of them are optimized upon a large number of external training dataset, which uses the fixed bicubic operation to downsample HR images for constructing training pairs. Similarly, in the test phase, the test images are down-sampled by the bicubic kernel before being feeding into the network. Then, the generated results are compared to Ground Truth (GT) in terms of PSNR, SSIM, and other metrics. The above deep learning based methods show significant results in the noise-free "bicubic" downsampling condition.

% \noindent
However, in real-world situations, the downsampling blur kernels are complicated and unavailable. As revealed in ~\cite{efrat2013accurate,yang2014single}, learning-based methods will suffer severe performance drops when the blur kernel in the test phase is different from that in the train phase. This kind of kernel mismatch will introduce undesired artifacts to output images. Thus, the problem with unknown blur kernels, also known as blind SR, has limited the application of most of deep learning based SR methods in real-world situations. To solve this limitation, many novel methods have been proposed. For instance, some blind SR methods~\cite{begin2004blind,he2011single,wang2005patch} are model-based, which introduce prior knowledge to the deep learning area and usually involve complicated optimization procedures. These methods do not calculate the SR kernel directly, but assume that SR networks are robust and transferable to variations in the downsampling kernels. 
% Because of their excellent mobility, they can compensate for the accuracy drop caused by the kernel mismatch but degrade the accuracy of models on common dataset that are generated by the "bicubic" kernel.
~\cite{michaeli2013nonparametric} exploits the recurrence of small image patches across scales of a single image to estimate the unknown SR kernel directly from the LR input image. However, it fails when the SR scale is larger than 2, and the runtime is very long. ZSSR~\cite{shocher2018zero} does not adopt the regular training process on the external datasets and trains from scratch for each test image, so that specific models pay more attention to information in the picture. Nevertheless, the runtime is greatly increased, limiting its application in the real scene. The current challenge is that in the above SR models, no one can show ideal performance simultaneously on both SISR and blind SR tasks. Thus, it's urgent to propose a SR method to  meet this challenge.
\begin{figure}
    \centering
    \subfigure
    {
    \begin{minipage}[b]{.4\linewidth}
        \centering
        \includegraphics[width=\textwidth]{shift.pdf}
        \caption{The 1x1 shift-conv}
        \label{fig:shift-conv}
    \end{minipage}
    }
    \subfigure
    {
    \begin{minipage}[b]{.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{ASA.pdf}
        \caption{The accelerated self-attention}
        \label{fig:ASA}
    \end{minipage}  
    }
\end{figure}

In this paper, to improve the poor performance of most Blind-SR models in noise-free ``bicubic" downsampling condition while boosting the extensibility of SISR models, we propose a novel framework ZHE LI XU YAO JIA SHANG FRAMEWORK DE MINGZI. On the one hand, inspired by the success of transformer-based methods in computer vision tasks, we build our model on top of the SOTA transformer-based Super-Resolution model SwinIR (light-weight version)~\cite{liang2021swinir} to enhance performance in the nosie-free "bicubic" downsampling condition. However, there are many redundant and fragmented components that are not efficient for the SR task. To save computation resources, we replace Residual Swin Transformer Block (RSTB) in SwinIR with Efficient Long-Range Attention Block (ELAB)~\cite{zhang2022efficient}, which consists of two parts, an extra local feature extraction module (ELF) and the deep feature extraction module (DF). In ELF, local structural information is efficiently extracted by two shift convolutions (shift-conv)~\cite{wu2018shift}, each of which has the same arithmetic complexity as an 1 $\times$ 1 convolution. For the self-attention calculation in DF, a group-wise multi-scale self-attention (GMSA)\cite{zhang2022efficient} operator is used to enlarge the receptive field. What's more, a shared attention mechanism\cite{zhang2022efficient} is exploited to reduce parameters. To compensate for the accuracy drop caused by the reduced number of parameters, we add deformable convolution~\cite{dai2017deformable}, which is light weight, to enlarge the receptive field. As it is based on the idea of augmenting the spatial sampling in the modules with additional offsets and learning the offsets from the target tasks, without introducing additional supervision. Recent studies~\cite{dai2021coatnet,graham2021levit,xiao2021early} suggest that using convolutions in early stages benefits the performance of Vision Transformers. Thus, we follow this design to add additional convolutions in early stages. Inspired by the intuition that the bottlenecks contain all the necessary information, and to improve the performance of our model, we finally choose the MBConv~\cite{sandler2018mobilenetv2}, where the inverted design is more memory efficient, as the convolution layer that we add.  
% 这里要写一下为啥使用mbconv和deformable conv
On the other hand, considering that the SISR models show poor performance in real-world applications, and conventional blind SR models such as ZSSR~\cite{shocher2018zero} usually avoids the training process on the external dataset but trains from scratch for each test image, we propose a new training recipe ZHE LI YAO QI YI GE training recipe DE MINGZI. We first pre-train our model on the external dataset, and then, an estimated blur kernel that can best preserve the distribution of patches across scales of the LR image is then generated by KernelGAN~\cite{bell2019blind}. We downsample the test image with the corresponding kernel (the estimated kernel) and synthesize an LR-$LR_{son}$ image pair, and then, fine-tune our model for several iterations. Finally, we feed a given test image to the model to get a super-resolution image. When transfer learning with the help of a large-scale external dataset is performed for our model, the performance of our model will obtain significant improvement. At the same time,it can boost the extensibility of our model in real-world situations. 

In summary, our overall contribution is four-fold:
% \renewcommand{\labelitemi}{\textbullet}
\begin{itemize}
    \item[\textbullet] For the real-world image characteristics, we propose a new method ZHE LI JIA SHANG METHOD DE MINGZI. In it, transfer-learning with the help of a large-scale external dataset is performed, and then, we can get a generalized and fast-adaption neural network, that can show good performance in SISR and blind SR tasks. 
    \item[\textbullet] We propose a light-weight transformer-based model for super resolution, which has a low parameter count and shows good performance in SISR tasks.
    \item[\textbullet] To boost the extensibility of our model in real-world situations, we further propose a new training recipe on top of our proposed model, where we first per-train our model and perform transfer-learning on the new dataset to take advantage of external and internal learning, realizing better performance and fast-adaption for real-world applications. 
    \item[\textbullet] experiment results
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{GMSA.pdf}
    \caption{The group-wise multi-scale self-attention}
    \label{fig:GMSA}
\end{figure}


==> method.tex <==
\section{Method}
In this section, we introduce a single-image blind super-resolution (SIBSR) framework, which consists of a light-weight transformer-based model and a novel training strategy, as shown in Figure\ref{fig:training_recipe}. With the proposed training strategy, the proposed model can achieve significant performance with a few backpropagation gradient updates and great scalability for the real-world applications. The learning pocess of the framework is mainly divided to two stages, call-level learning on the pre-train model and final-level fine-tune on real-world images. The first stage is to pre-train the porposed model on a large scale external dataset to guarantee its great performance on ideal downsampling condition and fast-adaption when the proposed model is extended to the real-world situations. The second stage is to boost the scalability of our model, achieving the usage in real-world situations.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{MBConv.pdf}
%     \caption{MBConv}
%     \label{fig:MBConv}
% \end{figure}

% our model is built on top of the SOTA transformer-based Super-Resolution model SwinIR and consists of three modules: shallow feature extraction, deep feature extraction, and high-quality image construction modules. Our purpose is to build a light-weight transformer-based super-resolution neural network. Thus, in the deep feature extraction module, we first replace RSTB with ELAB, but our experiments show that directly applying this vanilla method will lead accuracy drop. Based on this, we add two other modules to compensate for task accuracy
\subsection{Network Architecture}
As shown in Figure\ref{fig:architecture}, the proposed model contains three modules, shallow feature extraction module (SF), deep feature extraction module (DF) and high quality image reconstruction module (RC). In specific, given a low-resolution (LR) input I$_{LR}$\in \mathbb${R^{3{\times}H{\times}W}}$, where H and W are the height and width of the LR image, respectively, we first use the shallow feature extraction module denoted by H$_{SF}(\cdot)$, which only consists of a single 3$\times$3 convolution, to extract local feature I$_{local}$ \in \mathbb${R^{C{\times}H{\times}W}}$:
\begin{equation}
     I_{local} = H_{SF}(I_{LR}), 
\end{equation}
where C is the feature channel number.

I$_{local}$ then goes to the deep feature extraction module, denoted by H$_{DF}(\cdot)$. That is:
\begin{equation}
    I_{deep} = H_{DF}(I_{local}),
\end{equation}
where X$_d$ \in \mathbb${R^{C{\times}H{\times}W}}$ denotes the output of the deep feature extraction module. The deep feature extraction module consists of a mobile bottleneck convolution (MBConv), denoted by H$_{mbconv}$, N cascaded efficient long-range attention blocks (ELAB), denoted by H$_{ELAB}$, a deformable convolution (Deform Conv), denoted by H$_{deform}$ and a 3$\times$3 convolution. More specifically, intermediate features I$_{mbconv}$, I$_{deform}$, I$_1$, I$_2$, $\dots$, I$_N$, and the output deep feature I$_{deep}$ are extracted block by block as
\begin{equation}
    \begin{array}{rcl}
        I_{mbconv} &=& H_{mbconv}(I_{local}) \\
        I_i &=& H_{ELAB_i}(I_{i-1}),\qquad i=1,2, \dots, N \\
        I_{deform} &=& H_{deform}(I_N) \\
        I_{deep} &=& H_{CONV}(I_{deform}),
    \end{array}
\end{equation}
where H$_{ELAB_i}(\cdot)$ denotes the \emph{i}-th ELAB and H$_{CONV}$ is the last convolutional layer. Finally, taking I$_{deep}$ and I$_{local}$ as inputs, the HR image I$_{HQ}$ is reconstructed as:
\begin{equation}
    I_{RHQ} = H_{RC}(I_{deep} + I_{local}),
\end{equation}
where H$_{RC}$ is the reconstruction module. Here we choose a sub-pixel convolution layer~\cite{shi2016real} to upsample the feature. The proposed model can be optimized with the commonly used loss functions for SR, such as L$_2$~\cite{dong2015image, kim2016accurate, tai2017image, tai2017memnet} and L$_1$~\cite{lai2017deep, lim2017enhanced, zhang2018residual}. For simplicity, we choose L$_1$ as our loss function by minimizing the L$_1$ pixel loss.
% \begin{equation}
%     \mathcal{L} = \mid\mid I_{RHQ} - I_{HQ} \mid\mid_1
% \end{equation}

% Where I$_{RHQ}$ is the output of our model and I$_{HQ}$ is the corresponding ground-truth HQ image.

\subsubsection{ELAB}
Despite the great success of transformer on computer vision tasks, it greatly suffers from its explosive parameters and high computational complexity. Thus, inspired by ~\cite{zhang2022efficient}, to bulid a light-weight transformer-based model, we introduce ELAB to the deep feature extraction moudle of the proposed model. In ELAB, the regular multi-layer perception is replaced with two shift-conv~\cite{wu2018shift} with a simple ReLU activation. It can help enlarge the receptive field of the proposed model preliminarily, while sharing the same arithmetic complexity as two cascaded 1$\times$1 convolutions. Moreover, to significantly reduce parameters, the accelerated attention mechanism is utilized. In the self-attention calculation procedure, three independent 1$\times$1 convolutions, denoted by $\theta, \phi, \psi$, are employed to map the input feature X into three different feature maps. In this block, $\theta$ is set the same as $\phi$, which can save 1$\times$1 convolution in each self-attention. For compensating for performance drops caused by the reduced number of parameters, instead of the regular self-attention, the group-wise multi-scale self-attention (GMSA) is used. In GMSA, the input feature map X is split into K groups, in each group, denoted by \{X$_k$\}$^K_{k=1}$, then calculate self-attention on the k-th group of features using window size M$_k$. In this way, the channel number is $\frac{C}{K}$, it's flexible for GMSA to control K groups computational cost$\frac{2}{K}(\sum_{k}M^2_k)HWC$ by changing the window size. Furthermore, in self-attention part, some modifications are made to accelerate the calculation of self-attention. Firstly, batch normalization (BN)~\cite{ioffe2015batch} is utilized to boost the efficiency and replace layer normalization (LN), which will fragment the calculation into many element-wise inefficient operations.


On the other hand, in the self-attention part, given a feature map of C$\times$H$\times$W, the computational complexity of the window-based self-attention~\cite{liu2021swin,liang2021swinir} using M$\times$M non-overlapped windows is 2M$^2$HWC. The window size M determines the range of self-attention calculation, and a larger M can exploit more self-similarity information. However, directly enlarging M will increase the computational cost and resources. To make the network more efficient, the origin self-attention is replaced with group-wise multi-scale self-attention (GMSA). In GMSA, the input feature map X is split into K groups, in each group, denoted by \{X$_k$\}$^K_{k=1}$, then calculate self-attention on the k-th group of features using window size M$_k$. In this way, the channel number is $\frac{C}{K}$, it's flexible for GMSA to control K groups computational cost$\frac{2}{K}(\sum_{k}M^2_k)HWC$ by changing the window size. Furthermore, in self-attention part, some modifications are made to accelerate the calculation of self-attention. Firstly, batch normalization (BN)~\cite{ioffe2015batch} is utilized to boost the efficiency and replace layer normalization (LN), which will fragment the calculation into many element-wise inefficient operations. 

Secondly, in the self-attention calculation procedure, three independent 1$\times$1 convolutions, denoted by $\theta, \phi, \psi$, are employed to map the input feature X into three different feature maps. In this block, $\theta$ is set the same as $\phi$, which can save 1$\times$1 convolution in each self-attention. The above two modifications will alleviate the computation and memory cost of self-attention without sacrificing the self-attention performance.

Unlike RSTB in SwinIR, the block ELAB we used can remove the masking strategy and relative position bias. Although relative position bias can improve the performances, it makes models fragile to the resolution change~\cite{xie2021segformer}. Training with multi-scale images is an important capability of a model for detection and segmentation tasks. Thus, removing relative position bias can make the model more flexible to the input and boost the extensibility of the model to some extent. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{training recipe.pdf}
%     \caption{training recipe}
%     \label{fig:training_recipe}
% \end{figure}
\subsubsection{MBConv}
Depthwise Separable Convolutions, which is to replace a full convolutional operation, are a key building block for many efficient neural network architectures~\cite{howard2017mobilenets,chollet2017xception,zhang2018shufflenet}. In Depthwise Separate Convolutions, the full convolution is divided into two separate layers. The first layer is a depthwise convolution. It performs lightweight filtering by applying a single convolutional filter per input channel. The second layer is a pointwise convolution, which is 1$\times$1 convolution, and builds new features through computing linear combinations of the input channels. This can alleviate the computation and memory costs to a great extent. Thus, as shown in Figure\ref{fig:MBConv}, in this block based on the Depthwise Separate Convolutions, given an input, firstly, a 1$\times$1 convolution is performed to increase the dimension, and then followed by the depthwise convolution. Secondly, a squeeze-and-excitation optimization~\cite{hu2018squeeze} is added to enlarge the receptive field further, then followed by the pointwise convolution. Furthermore, the inverted design is more memory efficient which will further decrease running time and parameter count for bottleneck convolution. Inspired by the intuition that the bottlenecks contain all the necessary information, we apply this block to improve the performance for the accuracy drop caused by replacing the origin module with light-weight modules. 
\subsubsection{Deformable Convolution}
Considering the challenge that how to accommodate geometric variations or model geometric transformations in image scale and part deformation, there are two ways in general. The first is to build the training datasets with sufficient desired variations, but robust representations will be learned from data at the cost of resources and parameters. The second is to use transformation-invariant features and algorithms. However, there exists drawbacks in the above two ways. The geometric transformations are assumed fixed and known. Nevertheless, this assumption prevents generalization to new tasks possessing unknown geometric transformations. Therefore, to address these problems, the Deformable Conv is proposed. It adds 2D offsets to the regular grid sampling locations in the standard convolution. The offsets are learned from the preceding feature maps via additional convolution layers. Moreover, the Deformable Conv is light weight. It introduces small amount of parameters and computation for the offsets learning. Because of these properties, we add the Deformable Conv at the end of our network architecture to improve the performance further and make our model feasible to extend our model to test under a new resolution or train with multi-resolution.

\begin{figure}
    \centering
    \subfigure
    {
    \begin{minipage}[b]{.28\linewidth}
        \centering
        \includegraphics[width=\textwidth]{MBConv.pdf}
        \caption{The mobile-bottleneck convolution}
        \label{fig:MBConv}
    \end{minipage}
    }
    \subfigure
    {
    \begin{minipage}[b]{.65\linewidth}
        \centering
        \includegraphics[width=\textwidth]{training_recipe.pdf}
        \caption{The training recipe}
        \label{fig:training_recipe}
        
    \end{minipage}
    }
    % \includegraphics[width=\textwidth]{training_recipe.pdf}
\end{figure}
\subsection{Training Recipe}
To extend our model to applications in the real world, we propose a transfer-learning method. Here is the pipeline of our training recipe. Firstly we pre-train our model on the external dataset (noise-free "bicubic" dataset). In order not to deviate from the goal that we want to calculate the SR kernel to deal with Blind SR tasks, rather than just make our model robust to variations in the downscaling kernel, we need to estimate the SR kernel that best preserves the distribution of patches across scales of the LR image to compensate for the accuracy drop caused by the blur kernel mismatch. Based on the internal cross-scale recurrence property~\cite{zontak2011internal}, which can be used to estimate the unknown SR-kernel directly from the LR input image, we introduce "KernelGAN"~\cite{bell2019blind}, which combines this property with Deep-Learning. Its \emph{Generator} is trained to generate a downscaled image of the LR test image, such that its \emph{Discriminator} cannot distinguish between the patch distribution of the downscaled image and the origin. 

The diversity of the LR-HR relations within a single image is  significantly small, related to noise and blur kernel. Thus, given an LR real-world test image I$_{LR}$, we use the estimated blur kernel to generate the lower resolution image I$_{LRson}$, and synthesize them as a data pair LR-LR$_{son}$. Then, we use our pre-train model to generate the high-resolution version I$_{SR}$ of the I$_{LRson}$, and use L$_1$ loss with ADAM optimizer~\cite{kingma2014adam} to learn the residual between the high-resolution version I$_{SR}$ and I$_{LR}$. With the help of training with the external dataset and our modified modules that remove relative position bias from the backbone SwinIR and make our model feasible for training with the multi-scale resolution, the runtime can be drastically reduced. Thus, only 10 iterations are needed. We start with a learning rate of 2$\times$10$^{-2}$, and then, change to 1$\times$10$^{-2}$ when the iteration is not larger than 4, and keep  5$\times$10$^{-3}$ until the end. Finally, the method in ~\cite{lim2017enhanced}(which generates 8 different outputs for the 8 rotations+flips of the test image I, and then combines them) can improve the performance of our backbone SwinIR on SISR tasks. Moreover, we replace their mean with the median of these 8 outputs. We further combine it with the back-projection of ~\cite{irani1991improving}, so that each of the 8 output images goes through multiple iterations of the back-projection and the final correction of the median image can also be done through the back projection.

Note that what is different from ZSSR~\cite{shocher2018zero}, on the level of network architecture, compared to our transformer-based model, the backbone of ZSSR is a fully convolution network, because of our model inherently doing well on SISR tasks, our model can show a better performance than ZSSR. On the level of training recipe, ZSSR trains from scratch on the small dataset for implementing the super-resolution task, but we pre-train our model on the external dataset, and then, transfer-learning is performed on our model to extend our model to a new task. It makes our model fast-adaption on downstream tasks and real-world application and further boosts the accuracy of our model.

==> relate.tex <==
\section{Related Work}
\subsection{Single Image Super Resolution}
SISR is based on the image degradation model as
\begin{equation}
    I_{LR} = (I_{HR} \ast k_s)\downarrow_s
\end{equation}
where I$_{HR}$, I$_{LR}$, k$_s$, s denote HR, LR image, SR kernel and scaling factor, respectively. Recently, CNN-based methods~\cite{dong2016accelerating,shi2016real,lai2017deep,kim2016deeply,tai2017image} have demonstrated impressive peformance in the SR task. SRGAN~\cite{ledig2017photo} first introduces residual blocks into SR networks. EDSR~\cite{lim2017enhanced} also uses a deep residual network for training SR model but removes unnecessary batch normalization layer in residual block. Zhang \emph{et al}~\cite{zhang2018image} achieving better performances than EDSR by introducing the channel attention to residual block to form very deep network. Haris \emph{et al}~\cite{haris2018deep} propose deep back-projection networks to exploit iterative up and down sampling layers, providing an error feedback mechanism for projection errors at each stage. SRMD~\cite{zhang2018learning} propose a stretching strategy to integrate kernel and noise information to cope with multi degradation kernels in a SR network. The breakthrough of transformer networks in natural language processing(NLP) inspires researchers use Self-Attention(SA) in vision tasks. Thus, the transformer-based super-resolution models come to being. SwinIR~\cite{liang2021swinir} adapts the Swin Transformer~\cite{liu2021swin} to image restoration, which combines the advantage of both CNNs and transformers. ELAN~\cite{zhang2022efficient} bases on SwinIR removes redundant designs such as masking strategy and relative position encoding to make the network more efficient.

\subsection{Blind Super-Resolution}
Compared to SISR, Blind SR assumes that the degradation kernels are unknown. In real-world applications, the SR kernel of images are influenced by the sensor optics. In recent years, some Blind-SR methods~\cite{wang2005patch,joshi2008psf,he2011single} introduces prior into the deep learning area, however, these methods do not explicitly calculate the SR kernel, what they do is make their model more robust to variations. In contrast, Michaeli and Irani~\cite{michaeli2013nonparametric} estimates the kernel based on the recurrence of small image patches(5$\times$5, 7$\times$7) across scales of a single image but fails for SR scale factors larger than $\times$2. KernelGAN~\cite{bell2019blind} based on Interal-GAN~\cite{shocher2019ingan} estimates the SR kernel that best preserves the distribution of patches across scales of the LR image. ZSSR~\cite{shocher2018zero} abandons the training process on a big data but trains a small full convolution networks for each image from scratch to learn image specific internal structure. However, it requires thousands of backpropagation gradient updates at test time drasticly increasing the runtime.
